Characterizing Universal Reconfigurability of Modular Pivoting Robots

We give both efficient algorithms and hardness results for reconfiguring between two connected configurations of modules in the hexagonal grid. The reconfiguration moves that we consider are "pivots", where a hexagonal module rotates around a vertex shared with another module. Following prior work on modular robots, we define two natural sets of hexagon pivoting moves of increasing power: restricted and monkey moves. When we allow both moves, we present the first universal reconfiguration algorithm, which transforms between any two connected configurations using $O(n^3)$ monkey moves. This result strongly contrasts the analogous problem for squares, where there are rigid examples that do not have a single pivoting move preserving connectivity. On the other hand, if we only allow restricted moves, we prove that the reconfiguration problem becomes PSPACE-complete. Moreover, we show that, in contrast to hexagons, the reconfiguration problem for pivoting squares is PSPACE-complete regardless of the set of pivoting moves allowed. In the process, we strengthen the reduction framework of Demaine et al. [FUN'18] that we consider of independent interest.

==> oldStuff.tex <==
\mati{From here down we have old ideas that have been discarded}
\section{Old Attempt 2 at a constructive proof (using potential)}
The following algorithm seems to work and is nicely described. The problem is that we cannot prove it will terminate in subexponential time

\subsection{Defining the level}
Before we introduce our algorithm, we need to introduce the concept of {\em level} of a robot. Intuitively speaking, the level of a robot gives a measure of how easily a robot can reach the outer shell (the lower the level the easier it will be).

In the following, we assume that robots lie in a hexagonal grid with horizontal layout (i.e., two edges of each robot are vertical)\mati{todo: figures are actually using a vertical layout. We should update them (rotating them 90 degrees)...or redefine extremes based on x coordinates}.

Given a configuration $S$ of $n$ robots, the {\em level} is a function $\ell\colon S \rightarrow \mathbb{Z}$ that assigns a positive integer to each robot of $S$. let $r_0$ be the robot of lowest $y$-coordinate (and lowest $x$ coordinate in case of ties). We define $e_0=r_0$ and $e_1$ is the robot of highest $y$-coordinate in $S$. If there is a tie, we pick the robot that is furthest away (in the robot graph sense) from $e_0$. In case of further ties, we pick the robot of lowest $x$-coordinate.

If $e_1$ can move, we set the level of all robots in $S$ to be zero (that is $\ell(r)=0$ for all $r\in S$). Otherwise, we will set the level of some robots to be zero, and define remaining levels recursively.

Since $e_1$ has highest $y$-coordinate among all robots (and we break ties by $x$-coordinate), it must have 3 or more consecutive empty spaces around itself. Thus, the only reason why it cannot move is because it is a cut vertex. That is, the removal of $e_1$ would disconnect the configuration of robots into two components; let $R_0$ be the component containing $e_0$. We set the level of all robots of $R_0$ as zero and define  $S_1=S_0\setminus R_0$ as the remaining robots (note that $e_1\in S_1$ and robots in $S_1$ do not have a level assigned yet).

Now we continue with the process in a recursive fashion: starting from $i=1$, we define $e_{i+1}$ as a robot in $S_{i}$ with the largest difference in $y$ coordinates with $e_i$, in absolute value (as before, we break ties by distance to $e_i$, and further refining by smallest $x$-coordinate if needed ). Note that by construction, if $e_i$ was the robot of largest $y$-coordinate in $S_i$, then $e_{i+1}$ will be the one with smallest $y$-coordinate in $S_{i}$ (and {\em vice versa}). 

If $e_{i+1}$ can move (considering only robots in $S_{i}$ and ignoring those of lower level), we set the level of all robots in $S_{i}$ to be $i$ and we are done with the level definition. 

Otherwise, it must hold that $e_{i+1}$ is a cut vertex. Let $R_{i}$ be the connected component that would contain $e_i$ and $S_{i+1}=S_i\setminus R_i$. We define the level of all robots in $R_i$ as $i$. 

This process will continue until we find some level $i$ in which robot $e_{i+1}$ can move when we consider only the robots in $S_i$ (see an example in Figure~\ref{fig_levels}). 

\begin{figure}[tb]
\centering
\includegraphics[scale=0.3]{levels_example.png}
\caption{The configuration above has 5 levels. Level 0 is shown in purple, level 1 is shown in blue, level 2 is shown in green, level 3 is shown in brown, and level 4 is shown in red.}
\label{fig_levels}
\end{figure}

\begin{lemma}\label{lem_move}
$e_{\ell(S)}$ can move in $S$. Moreover, if $\ell(S)\geq 1$, it can become adjacent to a robot of level $j<\ell(S)$.
\end{lemma}
\begin{proof}
Note that, by definition of levels, we know that $e_{\ell(S)}$ can move in $S_{\ell(S)-1}$ (otherwise we would have one more level). Thus, we need to prove that the same robot can move when we consider all robots in the configuration. We show this by induction on the level $i$ of $S$. 

When $i=1$, we have $S_0=S$ and thus the statement is trivial. For larger values of $i$, we know that $e_{i+1}$ has three neighboring positions that contain no robot of $S_i$. Thus, in order to guarantee that $e_{i+1}$ can move, it to show that no robot of $S\setminus S_i$ can occupy these positions

The key lies in the fact that we only define $e_{i+1}$ when we know that $e_1,\ldots, e_i$ are a cut vertices. In particular, any path from $e_i$ to a robot of level $k\leq i$ must pass through $e_i$ (and in particular cannot be directly adjacent to $e_{k+1}$).

The second statement is shown as follows: consider the set of positions that $e_{\ell(S)}$ can move (which by Observation~\ref{obs_empty} is a cycle $C$). If the cycle contains $S$ in its interior, then $e_{\ell(S)}$ is in the outer shell (and thus $\ell(S)=0$). 

This cannot happen, and thus any robot that is adjacent to the cycle must do so on the outer face of $C$ interior of the cycle. In particular, there must exist at least one robot $r_1 \in S$ (resp., $r_2\in S$) that is adjacent to $C$ and has with higher (resp. lower) $y$-coordinate than any position of $C$. By definition of extreme points, it cannot happen that $\ell(r_1)=\ell(r_2)=\ell(e_{\ell(S)})$. Whichever robot with different level must have lower level, which is a witness of the statement.
\end{proof}


\subsection{Level properties}
We now give some interesting properties of the level. Given a configuration $S$ of $n$ robots, the {\em level} of $S$ is denoted by $\ell(S)$ and is the the highest level among all robots of $S$ (i.e., $\ell(S)=\max_{r\in S} \ell(r)$). Also, for any robot $r\in S$, let $y(r)$ denote the $y$-coordinate of $r$.

\begin{lemma}\label{lem_distinctycoords}
For any configuration $S$ of $n$ and $0<i< \ell(S)$ there is no robot in $S_i \setminus \{e_i\}$ that shares $y$ coordinate with $e_{i}$. In other words, $e_i$ is the unique robot in $S_i$ with highest or lowest $y$-coordinate.
\end{lemma}
\begin{proof}
Assume (for the sake of contradiction) that there exists a robot $r\in S_i\setminus \{ e_i \}$ such that $y(r)=y(e_i)$. 

Since $i$ is not the largest level, it follows that $e_i$ must be a cut vertex. Thus, $r \in S_i$ and $e_{i-1} \not\in S_i$. In particular, any path from $r$ to $e_{i-1}$ (in the dual graph) must pass through $e_i$. This implies that $d(e_{i-1},r)=d(r,e_i)+d(e_i,e_{i-1})>d(e_i,e_{i-1})$.

However, this is a contradiction on how we chose $e_i$ (both $r$ and $e_i$ have the same difference in $y$ coordinates with $e_{i-1}$, but $r$ is further away to $e_{i-1}$ than $r$).
\end{proof}

\begin{corollary}\label{cor_seq}
In any configuration $S$ of robots, the extreme points satisfy $y(e_0)\leq y(e_2)< y(e_4), \ldots < y(e_3)<y(e_1)$
\end{corollary}
Note that the inequality is not strict between $e_0$ and $e_2$, but it is strict in all other cases. Although we would like strict inequality everywhere, this cannot be avoided: in some cases the any choice of $e_0$ will lead to an $e_2$ with the same $y$-coordinate (see Figure~\ref{xxx}). \mati{put the M of McDonalds as example figure}).
\begin{figure}
    \centering
%    \includegraphics{macdonald.svg}
    \caption{There are two candidates for $r_0=e_0$. Whichever we pick will have the other one being $e_0$, and thus $y(r_0)=y(e_2)$. Making $e_0$ be a robot of highest coordinate will also lead to a  similar situation.}
    \label{fig:my_label}
\end{figure}

\begin{lemma}\label{lem_levels}
For any configuration $S$ of $n$ robots it holds that $\ell(S)<\sqrt{2n}$. 
\end{lemma}
\begin{proof}
Let $k=\ell(S)$. By corollary~\ref{cor_seq}, the difference in $y$ coordinates between $e_0$ and $e_1$ is at least $k-1$ (the $y$ coordinates from $e_1$ to $e_k$ must all be different). Since $S$ is connected, there must exist at least that many robots connecting them. Moreover, by definition of levels, those robots are of level $0$. By repeating the same argument between $e_1$ and $e_2$ we obtain at least $k-1$ different robots of level $1$ connecting them (recall that we could have $y(e_2)=y(e_0$).

For any $i>1$ we obtain a similar argument: the difference between $y(e_{i})$ and $y(e_{i+1})$ must be at least $k-i$ (since we know that robots $e_{i+2}, \ldots e_k$ must have $y$-coordinates in between them and all of those robots have different $y$-coordinate). Thus, we obtain that there are at least $k-i-1$ robots of level $i$ connecting $e_i$ and $e_{i+1}$

Summing up, in addition to the $k$ extreme robots, $S$ must contain at least $k-1$ robots of level 0, $k-1$ of level 1, $k-2$ of level 2, and so on. Combining this with the fact that $S$ has $n$ robots, we obtain the following bound on $k$.

\begin{eqnarray*}
k+(k-1)+(k-1)+\ldots+1 &\leq& n \\
(k-1)+\frac{k(k+1)}{2} &\leq& n \\
\frac{k^2}{2} &\leq& n \\
k&<&\sqrt{2n}
\end{eqnarray*}


%We prove the equivalent statement that to reach a recursive depth of $k$, we must have $n = \Omega(k^2)$. Because of the way we choose $e_{i+1}$, we decrease the height of the configuration by at least 1 every two times we recurse, and also get rid of a number of hexagons equal to at least the height of the configuration on every recursive call (since in $S \setminus S_i ?$ there must be a path from $e_i$ to $e_{i+1}$). So if a recursive depth of $k$ is reached, we know we've decreased the height at least $\frac{k}{2}$ times from our original configuration, and at each step have thrown away a number of hexagons bounded below by the height of that configuration. So if we reach a depth of $k$ we've thrown away at least $\sum_{i=1}^{\frac{k}{2}}i = \Omega(k^2)$ hexagons, so our original configuration contained at least $\Omega(k^2)$ hexagons.
\end{proof}
Note that the bound is asymptotically tight (see Figure~XXX)\mati{todo:add figure where we go sqrtn up, then sqrtn-1 down, and so on}.

\begin{corollary}
For any configuration $S$ of $n$ robots and $i\leq \ell(S)$ there are at least $\ell(S)-i$ many robots of level $i$. 
\end{corollary}
\mati{I do not think that the corollary is needed. We should also be able to deduce upper bounds (from the number of roots needed afterwards). Just putting it in case we may need it for a refined argument}

\subsection{Algorithm description}
With the level definition in place, we can now introduce our algorithm for universal reconfiguration. We follow the usual approach that transforms any configuration of robots into a specific canonical form (in our case, a collection of $n$ robots vertically aligned). Thus, any two configurations are connected by going via the canonical form (and executing one sequence of moves in reverse).


Our goal is to apply a sequence of {\em operations}. An operation is a fairly small sequence of robot moves with a clear goal (commonly to reduce the level of one or more robots). We start by introducing the simplest one.


\begin{definition}[Trivial operation]
This operation can be executed when there is a robot $r\neq r_0$ in the outer shell that can move. The {\em trivial operation} consists of making $r$ move by repeatedly moving clockwise until it places itself vertically under $r_0$ (effectively becoming the robot of lowest $y$-coordinate). 
\end{definition}
\mati{todo: add a figure of before/after the trivial operation}

Note that if robot $r$ did not start in the outer shell, $r$ cannot move, or $r=r_0$, then we say that the trivial operation cannot be executed on $r$.

Let $r$ be a robot of level $\ell(r)>0$ that can move but cannot execute a trivial operation. We introduce two alternative operations:

\begin{definition}[Singleton operation]
A singleton operation happens when $r$ can move to a place that is adjacent \textbf{only} to only robots of level $j$ (for some $j<\ell(r)$). If there are several candidate levels we place $r$ adjacent to the lowest possible level (if several locations are still possible, break ties lexicographically in the coordinates of the possible locations).
\end{definition}

\mati{todo: put figure before and after singleton operation. Make one in which the level of many robots grows so that it can be used afterwards in our discussion of potential. This can be achieved by having a tie in who was robot $e_i$.}

\begin{definition}[Cycle operation]
A cycle operation happens when $r$ can move to a new location that is adjacent to two robots of different levels. Let $j$ be the lowest of the two levels (note that $j<\ell(S)$). In case of ties, we break ties with the following priorities: first minimize the lowest possible level that $r$ becomes adjacent to, then the second level that $r$ becomes adjacent to. In case of further ties, just pick the lexicographically smallest coordinate position for $r$).
\end{definition}
\mati{todo: another pretty figure.}

\begin{lemma}\label{lem_oneinthree}
In any configuration of $n$ robots, we can always execute at least one of the three operations (trivial, singleton or cycle) on $e_{\ell(S)}$. Moreover, any operation can be executed in $O(n)$ moves.
\end{lemma}
\begin{proof}
First observe that if we cannot execute a trivial operation, then by definition it holds that $\ell(S)>0$. But in this case Lemma~\ref{lem_move}, robot $e_{\ell(S)+1}$ can move and be adjacent to robots of some lower level $j<\ell(S)$. If it is adjacent to only robots of level $j$ then it is a singleton operation. If it is adjacent to robots of another level other than $j$, then it will be a cycle operation. 

Note that $r$ cannot be placed adjacent to three robots of different levels at the same time (since these robots cannot be adjacent to each other, the only possibility is that the neighboring space of $r$ are empty, occupied, empty, and so on, but in this case $e_{\ell(S)+1}$ would not have been able move, which is a contradiction.
\end{proof}

Lemma~\ref{lem_oneinthree} is the basis of our algorithm: continuously apply operations until the configuration of robots is in the canonical form. Whenever more than one operation is possible, we choose the one that would make $e_{\ell(S)}$ adjacent to a robot of lowest possible level (in case of further ties we prioritize trivial over cycle over singleton).

After each operation we recompute the level of all robots. Note that this could potentially change the value of $\ell(S)$ and which robot becomes $e_{\ell(S)}$. 

In fact, a trivial operation will also change $r_0$ (the robot of lowest $y$-coordinate in the initial configuration). For simplicity in the exposition, rather than updating $r_0$ we simply ignore a robot $r$ once it executes a trivial operation and it places itself under $r_0$ (alternatively, we can force these robots to be of level $-1$ and all of our arguments also follow). This concludes the description of our algorithm.

\subsection{Termination}
The goal of this section is to show the following result.

\begin{theorem}\label{theo_terminat}
Hexagonal robots with the monkey move are universally reconfigurable. That is, we can transform starting connected configuration of $n$ hexagonal robots into another target configuration of $n$ robots by executing at most $O(n^{1+\sqrt{2n}})$ many moves.
\end{theorem}
Note, however that the bound on the number of moves is exponential. In the next sections we provide a modified algorithm to improve the number of moves needed.

We start by introducing a potential function. This function will help us show that all operations contribute towards termination of the algorithm. 

Given a configuration $S$ of $n$ robots, let $r_i= |\{r\in S \colon \ell(s)=i\}|$ be the number of robots of $S$ whose level is $i$. We also define $r_{-1}$ as the number of times that we have executed the trivial operation (or equivalently, the number of robots that have level $-1$). Recall that, by Lemma~\ref{lem_levels}, $S$ has at most $\sqrt{2n}$ many levels. The potential $\Phi$ of a configuration $S$ of $n$ robots is defined as the vector $\Phi(S)=(r_{-1},r_0,r_1, \ldots, r_{\sqrt{2n}})$.

Given two configurations $S_1$ and $S_2$ of robots, we say that $S_1$ has smaller potential if $\Phi(S_1)$ is lexicographically larger than $\Phi(S_1)$. \mati{todo: either put a figure or discuss past images. In one case all robots have level 0 and the potential is $(0,n,0,0,0,0,0,0)$. In the second case, potential is $(0,\sqrt{n},\sqrt{n}-1,\sqrt{n}-2,\ldots,1,0)$. The former is preferable because we can do a trivial operation, hence why lexicographically larger is decreasing potential.}

We now need to show that all three operations indeed lower the potential.

\begin{lemma}
The potential decreases after executing a trivial operation.
\end{lemma}
\begin{proof}
After we execute a trivial operation we increase the value of the first coordinate of the potential. Thus, regardless of any change in the other coordinates, we are getting a lexicographically larger potential vector (which is reduced potential). 
\end{proof}
\mati{Maybe this should be an observation? feels trivial to me}

Similarly, we want to show that potential decreases with the other two operations. We start by showing an intermediate result.

\begin{lemma}
The robot that moves in a singleton or cycle operation cannot become an extreme robot.
\end{lemma}
\begin{proof}
Say that we executed either of these operations and robot $r$ is adjacent only to robot(s) that were previously of level $j$ (if singleton operation) or robot(s) of level $j$ and $k>j$ (if cycle operation) for some $j>0$. 

Assume (for the sake of contradiction) that $r$ becomes an extreme robot after it has moved. Since $r$ attaches itself to a robot of level $j$, its $y$-coordinate can differ by $1$ to the robot it attaches to. In particular, it can only become $e_{j-2}$ or $e_j$ (other extreme robots must have larger difference in the $y$ coordinates with robots of $S_i$). In the former case, $r$ must have attached immediately above/below the former $e_j$ (note that in this case we must have $y(e_{j-2})=y(e_j)-1$). The latter case could also happen if $r$ is attached to another robot of level $j$ and the $y$ coordinate of its new position matches the $y$ coordinate of the former $e_j$. 

However, we clam that this is a contradiction. Indeed, in either of the two cases can only happens if $r$ can reach the outer shell of $S_i$. But if it can reach the outer shell of $S_i$, but repeatedly walking clockwise it must be able to reach a robot of level $j'<j$. This is a contradiction in the way we break ties in the operations (since we always try to go attach $r$ to the lowest possible level). 
\end{proof}

\begin{lemma}
The level of $e_{\ell(S)}$ decreases after executing a singleton operation. Moreover, only robots that were previously at level $\ell(S)$ can change their level.
\end{lemma}
\begin{proof}
\mati{TODO: observe that none of the only extreme robot that can change is $e_{\ell(S)}$. This is because when we do a singleton operation we cannot make a cycle and we cannot become extreme in $y$ coordinates.}
\end{proof}

Since we know that the level of $e_{\ell(S)}$ will decrease to some $j<\ell(S)$ and no robot of level $\ell(S)-1$ or smaller changes level, we get a lexicographic improvement in the potential.
\begin{corollary}
The potential decreases after executing a singleton operation.
\end{corollary}

\mati{Mental note: this is the case that makes the algorithm to be slowest. It seems to do local improvement, but our current analysis cannot prevent exponential bounds in runtime. For now we are focused in termination.}

Finally, we consider the cycle operation. 
\begin{lemma}
Consider a configuration of robots $S$ in which we have just executed a cycle operation connecting robots of level $i$ and $j$ (with $i<j$). The level of all robots $r\in S$ is either unchanged (if $\ell(r) \leq i$) or has been reduced to $i$ (otherwise).
\end{lemma}
\begin{proof}
\mati{TODO: We just need to show that we made a cycle containing $e_i$: on one hand we can reach the moved robot using only robots of level $i$, but on the other hand $e_i$ can reach $e_{i+1}, e_{i+2}, \ldots $ all the way to $e_j$. Because of the cycle (and definition of level), all robots drop their level to level $i$. Lower levels are unaffected as in previous cases}
\end{proof}

\begin{corollary}
In between two executions of trivial operations there are at most $O(n^{\sqrt{2n}})$ cycle and/or singleton operations.
\end{corollary}


This concludes the proof of Theorem~\ref{theo_terminat}. 



\subsection{Improving the bound on the number of moves}
\mati{Work in progress}


\pagebreak
\section{More old Definitions}
\mati{These are definitions that we copy/pasted. Just leaving in case we want to recycle at some point}

\begin{definition}{\textit{Extremal Robot.}}
A hexagon is extremal in some configuration if its $y$-coordinate is maximal or minimal.
\end{definition}

\emph{Note}. Extremal robots are either cut vertices or can move.\\


When there are multiple robots tied in the extreme direction we are looking in, we need to decide which one to pick.
We recurse when the topmost or bottommost robot is a cut vertex.\\
Candidate pick for extremal robot $e_{i+1}$ given extremal robot $e_i$ (a topmost robot):
Look at all robots of minimal $y$-coordinate (alternatively, look at maximal $y$-coordinate if $e_i$ was a bottommost robot) on the component of $e_i$. We call them candidate $C_1$, ... , $C_k$.
\begin{itemize}
\item Case 1: If any candidate $C_i$ is in a cycle, pick $e_{i+1}$ as any of them.  $C_i$ can move since it is not a cut vertex.
\item Case 2: Else, define metagraph $M$ with vertices $V=\{e_i,C_1,...,C_k\}$ and edge $ab\in M \iff \exists$ a path from $a$ to $b$ without passing through $V\setminus ab$.\\
Observation: The metagraph is a tree, otherwise some $C_i$ is in a metacycle. Then it is in a cycle which goes back to case 1.\\
Pick $e_{i+1}$ as any leaf.\\
Claim: when we yield($e_i$):
\begin{itemize}
\item Either $e_i$ (which is either top or bottom extremal on outer shell) moves
\item or generates yield($e_{i+1}$).
\end{itemize}
\end{itemize}


\begin{definition}{\textit{Base Robot.}}
Let the lowest $y$-coordinate robot be the base robot of a configuration. Call this hexagon $e_0$.
\end{definition}

The base robot can be any hexagon that has lowest $y$-coordinate - we don't care about ties. Let this robot be a part of component $0$, thus we define its {\em level}, to be $0$. Once we have set our base robot, we find the extremal robot that maximizes the $y$-coordinate. This seems somewhat ambiguous, as in our most recent example:

\begin{figure}[tb]
    \centering
    \includegraphics[width=.2\linewidth]{"cycle".png}
\end{figure}


\begin{definition}{\textit{Level.}}
Defining the levels of a given configuration is a recursive process. First find a bottommost robot $e_i$ (starting with $i=0$). This robot is a part of level $i$. To find the rest of the robots that are a part of level $i$, find the topmost robot $e_{i+1}$ (breaking ties if needed like defined in Definition 2.1). If $e_i$ and $e_{i+1}$ are on a cycle, or $e_{i+1}$ can move, then everything that hasn't been given a level is in level $i$. Else, virtually remove $e_{i+1}$ and every robot still connected to $e_i$ is in level $i$.\\
Remove level $i$ from the configuration, flip the configuration (so $e_{i+1}$ is now a bottommost robot), and do the recursive operation again. Keep recursing until all robots have been assigned a level.
\end{definition}

\begin{lemma}
Let $(C_i, e_i)$ be a rooted configuration at some recursion level $i$. Then, if $e_{i+1}$ can move, $\exists$ some position along the outer shell of $C_i$, such that $e_i$ is touching some level $C_j$, s.t. $j < i$.
\end{lemma}

\emph{Note.} The goal here is to find a position that is only touching $C_j$ and not $C_i$, that $e_{i+1}$ can get to. Thus we need one extra step after this lemma.

\section{Alternative proof 3: Universal Reconfiguration}
\mati{This is Oliver's original proof. Again it works, but we have no good bound for it}

Assume our hexagonal grid is oriented with horizontal lines (as shown in Figure~\ref{fig:top cut vertex}).

\begin{definition}{\textit{Outer Shell:}}
Given a connected configuration $C$, let $h$ be any hexagon in $C$ with maximum $y$-coordinate. Now imagine adding a new hexagon $g$ directly above (and facet-adjacent to) $h$. We define the ``outer shell'' of $C$ to be the set of positions reachable by pivoting $g$ without moving any hexagon in $C$.
\end{definition}
We will often abuse notation and say a hexagon $h \in C$ is on the outer shell of $C$ if it is contained in the outer shell of $C \setminus \{h\}$.

\begin{lemma} \label{lem:outer-shell}
If $h$ is on the outer shell of $C$ and $h$ is movable, pivoting $h$ counter-clockwise repeatedly will eventually bring $h$ back to its original position.
\end{lemma}
\begin{proof}
It is straightforward to check (by local case analysis) that for a hexagon on the outer shell to be obstructed from pivoting clockwise, it must also be obstructed from pivoting counterclockwise. Thus, if it can move at all, it can move in a cycle.
\end{proof}

\begin{definition}{\textit{Rooted Configuration:}}
We say $\langle C, h \rangle$ is a rooted configuration, with $h$ being the ``root'', provided $C$ is connected and $h$ is a hexagon in $C$ with minimum $y$-coordinate.
\end{definition}

\begin{theorem} \label{thm:rooted reconfiguration}
If $\langle C, h \rangle$ is a rooted configuration, there exists a sequence of pivots which never moves $h$ and which brings a movable hexagon (other than $h$) to the outer shell.
\end{theorem}

\begin{proof}
We prove by induction on the number of hexagons; the base case is trivial. Now, let $g$ be any hexagon in $C$ with maximum $y$ coordinate. Provided $|C| > 1$, $g \neq h$ by definition. If $g$ is not a cut vertex then it must be truly mobile, and on the outer shell, so we are done. Otherwise, $g$ is a cut vertex. For $g$ to be a hexagon of highest $y$-coordinate and a cut vertex, the only possible local configuration is that shown in Figure~\ref{fig:top cut vertex}. So $g$ is a cut vertex of degree 2. Let $B$ be the component in $C \setminus \{g\}$ not containing $h$, and let $C' = B \cup \{g\}$. Note that since $g$ has maximum $y$-coordinate in $C$, it must also have maximum $y$-coordinate in $C'$.

\begin{figure}[tb]
    \centering
    \includegraphics[width=.2\linewidth]{"top cut".pdf}
    \caption{The only possible local configuration in which a hexagon $g$ of maximum $y$-coordinate is also a cut-vertex. $g$ is shown in purple, and its neighbors in green; slots with red dots must be empty.}
    \label{fig:top cut vertex}
\end{figure}

Since $g$ has maximum $y$-coordinate in $C'$, if we rotate $C'$ by $180^{\circ}$ $g$ must have minimum $y$-coordinate, so $\langle C', g \rangle$ is a rooted configuration. Further, $\langle C', g \rangle$ must have fewer hexagons than $\langle C, h \rangle$: at the very least it doesn't contain $h$. So by our inductive hypothesis there exists a sequence of pivots that brings a hexagon to the outer shell of $C'$ without ever moving $g$. By Lemma~\ref{lem:outer-shell} a mobile hexagon on the outer shell can traverse the shell completely, so this sequence of pivots can be extended to roll such a mobile hexagon around the outer shell of $C'$ until it reaches $g$. Call this extended sequence of pivots $\Gamma$. 

We now examine how $\Gamma$ plays out when we return to considering $C'$ as a subconfiguration of $C$. Say $\Gamma$ can be carried out in $C$ without a pivot in $\Gamma$ ever being obstructed by a hexagon in $C \setminus C'$. So this mobile hexagon can be brought to one of the positions indicated with a red dot in Figure~\ref{fig:top cut vertex}. In any of the four cases, this hexagon is either mobile and on the outer shell, or causes $g$ to no longer be a cut vertex (making $g$ mobile and on the outer shell). Further, all of these moves use only hexagons which were originally in $C'$, and $h \notin C'$ by construction, so this would complete the proof of the inductive case.

On the other hand, say a hexagon in $C \setminus C'$ prevents a pivot in $\Gamma$ from occurring. Examine the first instance of such an obstruction; the pivot in question is either a standard pivot, or a monkey jump. If it is a standard pivot, with out loss of generality (up to rotation/reflection), it is of the form shown in Figure~\ref{fig:obstruction}. In this image, the purple hexagon is about to pivot to the spot marked with a red dot, by rotating about the green hexagon (both purple and green are in $C'$); however, $C \setminus C'$ obstructs this movement by filling one or more of the yellow slots. To see that every obstruction is of this form, first note that the pivoting hexagon cannot be $g$ since we took our pivot sequence to be one that never moves $g$. Further, $g$ is initially the only hexagon which is in $C'$ and also adjacent to a hexagon not in $C'$. Thus, since we are examining the \emph{first} time a hexagon not in $C'$ obstructs a pivot in $C'$, the moment before this pivot occurs, no hexagon in $C'$ other than $g$ touches a hexagon not in $C'$. So this means $v_1$ and $v_2$ cannot be occupied by a hexagon in $C \setminus C'$ since they would be touching purple, and they also cannot be occupied by hexagons in $C'$ since by assumption the pivot of purple to red is valid in $C'$. Now, if $v_3$ is occupied by a hexagon not in $C'$, purple can monkey jump to $v_2$ and become adjacent to $v_3$, and otherwise if $v_3$ is not occupied and $v_4$ is, purple can rotate into red and become adjacent to $v_4$. So in either case, we get a hexagon (purple) in $C' \setminus {g}$ to become facet adjacent to a hexagon in $C \setminus C'$. Now we consider the case where the first move in $C'$ blocked by a hexagon not in $C'$ is a monkey jump. Refer to Figure~\ref{fig:monkey}; in order for the monkey jump from purple to red across green to be obstructed, one of the yellow slots must be filled by a hexagon in $C \setminus C'$. But this would mean a hexagon in $C'$ other than $g$ is already adjacent to a hexagon in $C \setminus C'$, which we just argued cannot happen before the first obstruction. So a monkey jump in $C'$ cannot be the first move to be obstructed.

We have just shown that after the first obstruction, a hexagon in $C'$ other than $g$ becomes adjacent to a hexagon in $C \setminus C'$; call this hexagon $p$. If $p$ is still adjacent to some hexagon in $C'$, then this allows $g$ to move along the outer cycle: since $g$ was previously the only vertex connecting $C \setminus C'$ to $C'$ and $\Gamma$ preserved connectivity of $C \setminus C'$ and $C'$, any new connection between the two components must create a cycle incident on $g$, and so since $g$ is degree 2, it would cease to be a cut vertex. In the other case, if $p$ leaves $C'$ completely and becomes facet adjacent only to hexagons in $C \setminus C'$, then we have decreased the size of $C'$ by 1. So we can then continue applying our inductive hypothesis on the remaining hexagons in $C'$ (still using $g$ as the root); either at some point we will create a cycle incident on $g$ and thus allow $g$ to move along the outer cycle, or we will eventually decrease the size of $C'$ to 0, at which point $g$ becomes mobile. Thus in any case $g$ will eventually become mobile.

Since we chose $C'$ to be the component in $C \setminus \{g\}$ which did \emph{not} contain $h$, and all pivots performed occurred within $C'$, no pivot could ever have have moved $h$, thus completing the proof of the inductive case.

\begin{figure}[tb]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=.4\linewidth]{"obstruction".pdf}
		\subcaption{}
		\label{fig:obstruction}
	\end{minipage}%
		\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=.4\linewidth]{"monkey jump obstruction".pdf}
		\subcaption{}
		\label{fig:monkey}
	\end{minipage}
	\caption{(a) At least one of the yellow slots is filled by a hexagon in $C \setminus C'$, preventing the standard pivot of purple to red about green (purple and green are both in $C'$). (b) At least one of the yellow slots is filled by a hexagon in $C \setminus C'$, preventing purple from monkey jumping to red across the green hexagons (purple and both greens are in $C'$).}
	
	\label{fig:both obstructions}
\end{figure}

% At least one of the yellow slots is filled by a hexagon in $C \setminus C'$, preventing the pivot of purple to red about green (purple and green are both in $C'$).

% For a hexagon in $C \setminus C''$ to obstruct a monkey jump in $C'$ (purple jumps to red using greens), it would need to be in one of the yellow slots, and thus already be adjacent to $C'$.

\end{proof}

This immediately implies the following:

\begin{theorem}
Any configuration of hexagons can be reconfigured into any other using the standard pivot and monkey jump.
\end{theorem}
\begin{proof}
It suffices to show any configuration can be transformed to a vertical chain. Start by identifying any root of the configuration $h$. Now apply Theorem~\ref{thm:rooted reconfiguration} to get a hexagon to the outer shell, and roll it around the shell until it extends below $h$ (this is possible by Lemma~\ref{lem:outer-shell}). We then repeat this again and again, each time ignoring the chain of hexagons hanging below $h$; since Theorem~\ref{thm:rooted reconfiguration} says we can get a hexagon to the outer shell without ever moving $h$, the hexagons below $h$ have no effect. Eventually this process terminates in a vertical chain with $h$ at the top.
\end{proof}

